From local to global determinacy in concurrent graph games

In general, finite concurrent two-player reachability games are only determined in a weak sense: the supremum probability to win can be approached via stochastic strategies, but cannot be realized. We introduce a class of concurrent games that are determined in a much stronger sense, and in a way, it is the larger class with this property. To this end, we introduce the notion of \emph{local interaction} at a state of a graph game: it is a \emph{game form} whose outcomes (i.e. a table whose entries) are the next states, which depend on the concurrent actions of the players. By definition, a game form is \emph{determined} iff it always yields games that are determined via deterministic strategies when used as a local interaction in a Nature-free, one-shot reachability game. We show that if all the local interactions of a graph game with Borel objective are determined game forms, the game itself is determined: if Nature does not play, one player has a winning strategy; if Nature plays, both players have deterministic strategies that maximize the probability to win. This constitutes a clear-cut separation: either a game form behaves poorly already when used alone with basic objectives, or it behaves well even when used together with other well-behaved game forms and complex objectives. Existing results for positional and finite-memory determinacy in turn-based games are extended this way to concurrent games with determined local interactions (CG-DLI).

==> Tex/Conclusion.tex <==
%!TeX.root = ../main.tex
We have proved a general transfer result and provided four applications. Other possible applications include, e.g., the positional determinacy of locally determined concurrent parity games (on infinite graphs as in \cite{zielonka1998infinite}), mean-payoff games on finite graphs \cite{ehrenfeucht1979positional}, etc. Also, our transfer result with deterministic Nature combines well with another transfer result from \cite{DBLP:journals/mlq/Roux14} to obtain Nash
equilibria. We mention two examples of applications.
\begin{itemize}
	\item Two-player games with determined local interactions, finitely
	many outcomes, and Borel-measurable outcome assignments have Nash
	equilibria;
	\item Two-player priority games (i.e. multi-outcome parity-like games)
	with determined local interactions have positional Nash equilibria.
\end{itemize}
The proofs, not typeset as of now, share many similarities with the proofs of Corollaries \cite[3.4 and 3.8]{DBLP:journals/mlq/Roux14}, respectively.

Note that two recent articles provide results where winning in some
concurrent graph games may be achieved via deterministic strategies:
\cite{DBLP:conf/concur/AghajohariAH19}, where bidding takes place at each vertex for the control of the vertex, and \cite{DBLP:conf/mfcs/Roux18}, where deterministic strategies suffice to win for one player, and memoryless uniform stochastic strategies suffice for the other player. The three results are incomparable in strength, primarily because they look at different facets of concurrency.

% (Further note that the terminology ``local determinacy'' occurs in
% \cite{DBLP:conf/concur/AghajohariAH19} to mean something similar but 
%different,
% which takes the
% objective into account, not just the arena.)

==> Tex/DeterminacyEquiv.tex <==
Consider a concurrent graph arena $\Aconc = \AcoloredConc$ %that is locally determined
, and its sequential version, the turn-based graph arena $\ATurnConc = \AcoloredSeq$. In the rest of this section, we prove a determinacy equivalence between $\Aconc$ and $\ATurnConc$ when $\Aconc$ is locally determined. %This will allow us to prove determinacy results on concurrent graph arenas that are locally determined by using well-known results on determinacy of turn-based graph arenas. %In the rest of this section, the function $\OneTwo{V}{Q}: \starom{V} \rightarrow \starom{Q}$ will be abbreviated $\OneTwoQ$.

First, let us consider the sets of compatible paths $\OutA{\omega}{\Aconc}(\s)$ with a strategy $\s$ in a concurrent graph game $\Games{\Aconc}{W}$ and the sets of compatible paths $\OutA{\omega}{\ATurnConc}(\sigma)$ with a strategy $\sigma$ in its sequential version $\Games{\ATurnConc}{W^\Aconc}$. More specifically, let us compare the two sets $\OutA{\omega}{\Aconc}(\s)$ and $\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$ for the inclusion. Interestingly, if one is included in the other, then this implies that if a strategy is winning in one arena, then the other also is in the other arena. Formally, we have the following lemma: 
\begin{lemma} 
	Consider a strategy $\s$ in a game $\Games{\Aconc}{W}$ and a strategy $\sigma$ in its sequential version $\Games{\ATurnConc}{W^\Aconc}$ for the same Player (whether it is $\A$ or $\B$).
	\begin{itemize}
		\item Let us assume that $\OutA{\omega}{\Aconc}(\s) \subseteq \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$. If $\sigma$ is a winning strategy in the game $\Games{\ATurnConc}{W^\Aconc}$, then so is $\s$ in the game $\Games{\Aconc}{W}$;
		\item Let us assume that  $\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)] \subseteq \OutA{\omega}{\Aconc}(\s)$. If $\s$ is a winning strategy in the game $\Games{\Aconc}{W}$, then so is $\sigma$ in the game $\Games{\ATurnConc}{W^\Aconc}$.
		\label{lem:inclusion_outcome_win}
	\end{itemize}
\end{lemma}
\begin{proof}[Proof sketch.]
	We prove this results in the case of strategies for Player $\A$ %(the other case is analogous)
	. Recall that $U_Q = \inv{\extendFunc{\colFunc}}[W]$ and $U_V = \inv{\extendFunc{\colFunc_\Aconc}}[W^\Aconc]$. Let $\projec{V}{Q}' = \restr{\projec{V}{Q}}{\OutStrat{\ATurnConc}^\omega}$. Then, we have $U_V = \inv{\projec{V}{Q}'}[U_Q]$.
	
	Now, assume that $\OutA{\omega}{\Aconc}(\s) \subseteq \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$. If $\sigma$ is a winning strategy for Player $\A$ in $\Games{\ATurnConc}{W^\Aconc}$, we have $\OutA{\omega}{\ATurnConc}(\sigma) \subseteq U_V$, hence%by Observation~\ref{obs:even_ind_surj}
	: $\OutA{\omega}{\Aconc}(\s) \subseteq \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)] \subseteq \projec{V}{Q}[U_V] \subseteq U_Q$ %(it is, in fact, an equality since the function $\projec{V}{Q}$ is surjective)
	. Thus, $\s$ is a winning strategy for Player $\A$ in the game $\Games{\Aconc}{W}$. 
	
	Now, assume that $\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)] \subseteq \OutA{\omega}{\Aconc}(\s)$. If $\s$ is a winning strategy for Player $\A$ in the game $\Games{\Aconc}{W}$, we have $\OutA{\omega}{\Aconc}(\s) \subseteq U_Q$, hence%, by Observation~\ref{obs:even_ind_surj}
	: $\OutA{\omega}{\ATurnConc}(\sigma) \subseteq \inv{\projec{V}{Q}'}[\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]] \subseteq \inv{\projec{V}{Q}'}[\OutA{\omega}{\Aconc}(\s)] \subseteq \inv{\projec{V}{Q}'}[U_Q] = U_V$.	Thus, $\sigma$ is a winning strategy for Player $\A$ in the game $\Games{\ATurnConc}{W^\Aconc}$.
	%\vspace*{-10pt}
\end{proof}
\begin{proof}
	We prove the two points in the case of strategies for Player $\A$ (the other case is analogous). Recall that we have $U_Q = \inv{\extendFunc{\colFunc}}[W]$ and $U_V = \inv{\extendFunc{\colFunc_\Aconc}}[W^\Aconc]$. Let us denote by $\projec{V}{Q}' = \restr{\projec{V}{Q}}{\OutStrat{\ATurnConc}^\omega}$ the restriction of the function $\projec{V}{Q}$ to paths in the turn-based game $\ATurnConc$. Then, by definition of the function $\colFunc_\Aconc$, we have $\projec{\colSetSeq}{\colSet} \circ \extendFunc{\colFunc_\Aconc} = \extendFunc{\colFunc} \circ \projec{V}{Q}'(\pi)$. It follows that, $U_V = \inv{\extendFunc{
	\colFunc_\Aconc}}[W_\Aconc] = \inv{\extendFunc{
	\colFunc_\Aconc}}[\inv{\projec{\colSetSeq}{\colSet}}[W]] =  \inv{(\projec{\colSetSeq}{\colSet} \circ \extendFunc{\colFunc_\Aconc})}[W] = \inv{(\extendFunc{\colFunc} \circ \projec{V}{Q}')}[W] = \inv{\projec{V}{Q}'}[\inv{\extendFunc{\colFunc}}[W]] = \inv{\projec{V}{Q}'}[U_Q]$.
	
	Now, assume that $\OutA{\omega}{\Aconc}(\s) \subseteq \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$. If $\sigma$ is a winning strategy for Player $\A$ in $\Games{\ATurnConc}{W^\Aconc}$, we have $\OutA{\omega}{\ATurnConc}(\sigma) \subseteq U_V$, hence%by Observation~\ref{obs:even_ind_surj}
	: $\OutA{\omega}{\Aconc}(\s) \subseteq \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)] \subseteq \projec{V}{Q}[U_V] \subseteq U_Q$ %(it is, in fact, an equality since the function $\projec{V}{Q}$ is surjective)
	. Thus, $\s$ is a winning strategy for Player $\A$ in the game $\Games{\Aconc}{W}$. 
	
	Now, assume that $\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)] \subseteq \OutA{\omega}{\Aconc}(\s)$. If $\s$ is a winning strategy for Player $\A$ in the game $\Games{\Aconc}{W}$, we have $\OutA{\omega}{\Aconc}(\s) \subseteq U_Q$, hence%, by Observation~\ref{obs:even_ind_surj}
	: $\OutA{\omega}{\ATurnConc}(\sigma) \subseteq \inv{\projec{V}{Q}'}[\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]] \subseteq \inv{\projec{V}{Q}'}[\OutA{\omega}{\Aconc}(\s)] \subseteq \inv{\projec{V}{Q}'}[U_Q] = U_V$.	Thus, $\sigma$ is a winning strategy for Player $\A$ in the game $\Games{\ATurnConc}{W^\Aconc}$.
	%\vspace*{-10pt}
\end{proof}
\pbcomment{Preuve précédente: ne pas inclure dans la version conf}

Now, we examine how one can translate a strategy in one arena into a strategy in the other arena while ensuring an inclusion of their outcome so that we can use Lemma~\ref{lem:inclusion_outcome_win}.

Let us first consider the simpler case where we translate strategies from the concurrent arena into strategies in its sequential version. for a strategy $\s \in \SetStrat{\Aconc}{\kappa}$ in a concurrent arena $\Aconc$, we consider the strategy $\sigma$ in $\ATurnConc$ such that, for $\pi \in \OutStrat{\Aturn}^*$, we have $\sigma(\rho) = \transSeq(\head(\pi),s(\projec{V}{Q}(\pi)))$. That is, $\sigma$ chooses as next state what would have happened in the concurrent arena if the strategy $\s$ were played on the projection of $\pi$ on $Q$. More formally, we have the following lemma:
\begin{lemma}
	Let $\Aconc$ be a concurrent arena and $\s \in \SetStrat{\Aconc}{\kappa}$ be a strategy for Player $\kappa \in \{ \A, \B \}$. Then, $\sigma = \transSeq \circ (\head,\s \circ \projec{V}{Q}) \in \SetStrat{\ATurnConc}{\kappa}$ is a strategy for Player $\kappa$ in $\ATurnConc$ ensuring: $\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)] \subseteq \OutA{\omega}{\Aconc}(\s)$.
	\label{lem:conc_to_turn}
\end{lemma}
%\vspace*{-20pt}
\begin{proof}[Proof sketch.]
	We prove the result for Player $\B$. First, for all $\rho \cdot (q,\Succq{q})\in V^* \cdot V_\B$, one can check that $((q,\Succq{q}),\delta(q,a,b)) \in E_\B$. Therefore, $\sigma$ is in fact a strategy for Player $\B$.
	
	Now, consider an infinite path $\pi = \projec{V}{Q}(\pi') \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$. Let $i \geq 0$. We have $\pi_i = \pi'_{2 i} \in V_\A$. Hence,
	$\pi'_{2i+1} = (\pi'_{2i},\Succq{\pi'_{2i}}) \in V_B$. Then, $\pi'_{2i+2} = \sigma(\pi'_{\leq 2i+1}) = \delta(\pi'_{2i},a,b)$ for $b = \s \circ \projec{V}{Q}(\pi'_{\leq 2i+1}) = \s(\pi_{\leq i})$ and some $a \in A$ ensuring $\delta(\pi'_{2i},a,B) = \Succq{\pi'_{2i}}$. That is $\pi_{i+1} = \pi'_{2i+2} = \delta(\pi_{i},a,\s(\pi_{\leq i})) \in \delta(\pi_{i},A,\s(\pi_{\leq i}))$. %This holds for all $i \geq 0$.
	It follows that, $\pi \in \OutA{\omega}{\Aconc}(\s)$.	
	%	$\pi'_{2i+1} = \sigma(\pi'_{\leq 2i}) = (\head(\pi'_{\leq 2i}),\s \circ \projec{V}{Q}(\pi'_{\leq 2i})) = (\pi_i,\s(\pi_{\leq i}))$. Furthermore, since $(\pi'_{2i+1},\pi'_{2i+2}) \in E_\B$, we have $\pi'_{2i+2} \in \delta(\head(\pi'_{\leq 2i}),\s \circ \projec{V}{Q}(\pi'_{\leq 2i}),B) = \delta(\pi_{i},\s(\pi_{\leq i}),B)$. Since $\pi_{i+1} = \pi'_{2i+2}$, it follows that $\pi_{i+1} = \delta(\pi_{i},\s(\pi_{\leq i}),B)$. This holds for all $i \geq 0$. Hence, $\pi \in \OutA{\omega}{\Aconc}(\s)$.
\end{proof}
\begin{proof}
	We prove the result for Player $\B$ (the case of Player $\A$ is analogous). First, for all $\rho \cdot (q,\Succq{q})\in V^* \cdot V_\B$, we have $\sigma(\rho \cdot (q,\Succq{q})) = \transSeq \circ (\head,\s \circ \projec{V}{Q})(\rho \cdot (q,\Succq{q})) = \delta(q,a,b) \in V_\A$ for some $a \in A$ ensuring $\Succq{q} = \delta(q,a,B)$ and $b = \s \circ \projec{V}{Q}(\rho \cdot (q,\Succq{q})) \in B$. Hence, $((q,\Succq{q}),\delta(q,a,b)) \in E_\B$. That is, $\sigma$ is in fact a strategy for Player $\B$.
	
	Now, consider an infinite path $\pi = \projec{V}{Q}(\pi') \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$. Let $i \geq 0$. We have $\pi_i = \pi'_{2 i} \in V_\A$. Hence,
	$\pi'_{2i+1} = (\pi'_{2i},\Succq{\pi'_{2i}}) \in V_B$. Then, $\pi'_{2i+2} = \sigma(\pi'_{\leq 2i+1}) = \delta(\pi'_{2i},a,b)$ for $b = \s \circ \projec{V}{Q}(\pi'_{\leq 2i+1}) = \s(\pi_{\leq i})$ and some $a \in A$ ensuring $\delta(\pi'_{2i},a,B) = \Succq{\pi'_{2i}}$. That is $\pi'_{2i+2} = \delta(\pi_{i},a,\s(\pi_{\leq i}))$. Since $\pi_{i+1} = \pi'_{2i+2}$, it follows that $\pi_{i+1} \in \delta(\pi_{i},A,\s(\pi_{\leq i}))$. This holds for all $i \geq 0$. Hence, $\pi \in \OutA{\omega}{\Aconc}(\s)$.	
%	$\pi'_{2i+1} = \sigma(\pi'_{\leq 2i}) = (\head(\pi'_{\leq 2i}),\s \circ \projec{V}{Q}(\pi'_{\leq 2i})) = (\pi_i,\s(\pi_{\leq i}))$. Furthermore, since $(\pi'_{2i+1},\pi'_{2i+2}) \in E_\B$, we have $\pi'_{2i+2} \in \delta(\head(\pi'_{\leq 2i}),\s \circ \projec{V}{Q}(\pi'_{\leq 2i}),B) = \delta(\pi_{i},\s(\pi_{\leq i}),B)$. Since $\pi_{i+1} = \pi'_{2i+2}$, it follows that $\pi_{i+1} = \delta(\pi_{i},\s(\pi_{\leq i}),B)$. This holds for all $i \geq 0$. Hence, $\pi \in \OutA{\omega}{\Aconc}(\s)$.
\end{proof}

Let us now consider how to translate strategies from the sequential version of a concurrent game to that concurrent game. First, let us focus on strategies for Player $\A$, where the translation is easier since, informally, Player $A$ has the same amount of information in the concurrent game than in its sequential version. We establish the following lemma.
\begin{lemma}
	Let $\Aconc$ be a concurrent arena and $\sigma \in \SetStrat{\ATurnConc}{\A}$ be a strategy for Player $\A$ in the sequential version $\ATurnConc$. Then, there exists a strategy $\s \in \SetStrat{\Aconc}{\A}$ for Player $\A$ in the concurrent arena $\Aconc$ ensuring: $\OutA{\omega}{\Aconc}(\s) \subseteq \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
	\label{lem:turn_to_conc_A}
\end{lemma}
To prove this lemma, we consider the set $\OutA{+}{\ATurnConc}(\sigma)$ of finite paths compatible with the strategy $\sigma$ in $\ATurnConc$. Then, we define the function $\ext_\A: \projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)] \rightarrow \OutA{+}{\ATurnConc}(\sigma)$ in the following way: $\ext_\A(q_0) = q_0$ and $\ext_\A(\pi \cdot q) = \ext_\A(\pi) \cdot (\head(\pi),\sigma(\ext_\A(\pi))) \cdot q$. Note that, for all $\pi \in \projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]$, we have $\projec{V}{Q} \circ \ext_\A(\pi) = \pi$. %Let us proceed to the proof of this lemma.

\begin{proof}
	%$\s = \projTwo \circ \sigma \circ \ext_\A \in \SetStrat{\Aconc}{\A}$ for Player $\A$ in the concurrent arena $\Aconc$ where $\projTwo: V_A \rightarrow A$ such that for all $(q,a) \in V_A$, we have $\projTwo(q,a) = a$.
	
	We define the strategy $\s \in \SetStrat{\Aconc}{\A}$ for Player $\A$ in the concurrent arena $\Aconc$ such that for all $\pi \in \projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]$, we have $\s(\pi) = a$ where $a = \min_{<_A} \{ a' \in A \mid (\head(\pi),\delta(\head(\pi),a,B)) = \sigma(\ext_\A(\pi)) \} \neq \emptyset$ by definition of $E_\A$. %$\restr{s}{\projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]} = \projTwo \circ \sigma \circ \ext_\A$% where $\projTwo: V_\B \rightarrow A$ is such that $\projTwo((q,a)) = a$ for all $(q,a) \in V_\B$
	%, for all $\pi \in \projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]$, we have $\s(\pi) = a$ where $\sigma(\ext_\A(\pi)) = (\head(\pi),a)$ and $\s$ is defined arbitrarily on paths not in $\projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]$. 
	Now, consider $\pi \in \OutA{\omega}{\Aconc}(\s)$ and let us prove that, for all $i \geq 0$ we have $\pi_{\leq i} \in \projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]$. Let us proceed by induction. We have $\pi_{\leq 0} = q_0 \in \projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]$. Let us now assume that $\pi_{\leq i} \in \projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]$ for some $i \geq 0$. Then, $\s(\pi_{\leq i}) = a$ where $\sigma(\ext_\A(\pi_{\leq i})) = (\pi_i,\delta(\pi_i,a,B))$. Thus, we have $\pi_{i+1} \in \delta(\pi_i,a,B)$. Hence, $((\pi_i,\delta(\pi_i,a,B)),\pi_{i+1}) \in E_\B$. That is, $\ext_\A(\pi_{\leq i}) \cdot (\pi_i,\delta(\pi_i,a,B)) \cdot \pi_{i+1} \in \OutA{+}{\ATurnConc}(\sigma)$ and $\projec{V}{Q}(\ext_\A(\pi_{\leq i}) \cdot (\pi_i,\delta(\pi_i,a,B)) \cdot \pi_{i+1}) = \projec{V}{Q}(\ext_\A(\pi_{\leq i})) \cdot \pi_{i+1} = \pi_{\leq i} \cdot \pi_{i+1} = \pi_{\leq i+1}$. Therefore, $\pi_{\leq i+1} \in \projec{V}{Q}[\OutA{+}{\ATurnConc}(\sigma)]$.
	
	It follows that the infinite paths $\pi' \in V^\omega$ with $\{ \ext_\A(\pi_{\leq i}) \mid i \geq 0 \}$ as prefixes ensures: $\pi' \in \OutA{\omega}{\ATurnConc}(\sigma)$ and $\projec{V}{Q}(\pi') = \pi$. That is, $\pi \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
\end{proof}
\pbcomment{Pas dans la version conf}

Let us now consider strategies for Player $\B$. This case is trickier than the previous one as Player $\B$ has more information in the turn-based game $\ATurnConc$ since he knows the action chosen by Player $\A$ before playing, which is not the case in the concurrent game $\Aconc$. In fact,
we will assume in the following that the concurrent game we consider is locally determined.%the translation of strategy for Player $\B$ uses the local determinacy hypothesis, that was not used in the two previous proofs of Lemma~\ref{lem:conc_to_turn} and~\ref{lem:turn_to_conc_A}. 
We explain our construction on an example. 

\begin{figure}
	\begin{minipage}[b]{0.44\linewidth}
		\centering
		\includegraphics[scale=1]{Tex/Figure/ExampleTransfoStrat_Turn.pdf}     
	\end{minipage}
	\begin{minipage}[b]{0.23\linewidth}
		\centering
		\includegraphics[scale=1]{Tex/Figure/ExampleTransfoStrat_Interaction.pdf}   
		{\color{white} a} \newline
		{\color{white} a} \newline
	\end{minipage}
	\begin{minipage}[b]{0.25\linewidth}
		\centering
		\includegraphics[scale=1]{Tex/Figure/ExampleTransfoStrat_Conc.pdf}  
	\end{minipage}
	\caption{On the left hand side, we have a portion of a turn-based graph arena %of Figure~\ref{fig:unfold_concurrent}
	, with all the states reachable in at most two moves from the state $q$. This turn-based arena corresponds to the sequentialization of the portion of the concurrent arena on the right hand side (the edge between $q$ and $z$ is omitted as it is not available if Player $\B$ chooses the second column) with the local interaction in the state $q$ represented in the middle: it is the game form $I_3$ from Figure~\ref{fig:examples_game_forms}. Here, we have $A = \{ a_1,a_2,a_3 \}$ and $B = \{ b_1,b_2,b_3 \}$. A %(portion of a) 
	strategy for Player $\B$ is represented in blue arrows in the turn-based arena, with the states reachable with that strategy represented in blue. In the local interaction in the middle, these states are also colored in blue, whereas $z$ is in red. Finally, in the concurrent arena, the red states are the state reachable if Player $\B$ opts for the second row, which is the winning strategy for Player $\B$ in the win/lose game obtained from the game form $I_3$ if she has $\{ x,z \}$ as winning set.}
	\label{fig:transfo_strat_det}
\end{figure}
\begin{example}
	We want to translate a strategy into a concurrent arena from its sequential version while ensuring that every state reachable with that new strategy is also reachable in the sequential version with the original strategy. Consider the example of the strategy depicted in the left-hand side of Figure~\ref{fig:transfo_strat_det} from the state $q$. For each possible choices of Player $A$ (which corresponds to the rows of the local interaction), Player $\B$ reacts with his strategy and either $x$ or $y$ is reached. Then, we must exhibit an action for Player $\B$ to play in the concurrent game in state $q$ (which corresponds to a column in the local interaction) so that only the states $x$ and $y$ can be reached. To choose this action, we consider the local interaction $I_3$. We know that for each action of Player $\A$, there is one for Player $\B$ to reach the set $\{ x,y \}$ (it is given by the strategy depicted in the turn-based arena). It follows that Player $\A$ has no winning strategy in the win/lose game $I_3$ with $\{ x,y \}$ has winning set for Player $\B$. Since the local interaction $I_3$ is determined, Player $\B$ has a winning strategy in that win/lose game which is a strategy that ensures reaching a state not in %$\{ z \}$, that is reaching 
	$\{ x,y \}$. By opting for this strategy, which corresponds to choosing the second column in the local interaction, it follows that the states reachable in the concurrent arena from $q$ are $\{ x,y \}$ (depicted in red).
\end{example}

Let us formally establish a lemma stating that a strategy for Player $\B$ in the sequential version of a locally determined concurrent game can be translated into a strategy for Player $\B$ in that concurrent game while preserving an inclusion so that the result of Lemma~\ref{lem:inclusion_outcome_win} can be used.
\begin{lemma}
	Let $\Aconc$ be a locally determined concurrent arena and $\sigma \in \SetStrat{\ATurnConc}{\B}$ be a strategy for Player $\B$ in the sequential version $\ATurnConc$. Then, there exists a strategy $\s \in \SetStrat{\Aconc}{\B}$ for Player $\B$ in the concurrent arena $\Aconc$ ensuring: $\OutA{\omega}{\Aconc}(\s) \subseteq \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
	\label{lem:turn_to_conc_B}
\end{lemma}

%Similarly to the proof of Lemma~\ref{lem:turn_to_conc_A}, we consider the set $\OutA{+}{\ATurnConc}(\sigma)$ of finite paths compatible with the strategy $\sigma$ in $\ATurnConc$. 
\begin{proof}[Proof sketch.]
	The strategy $\s \in \SetStrat{\Aconc}{\B}$ is inductively defined on the set of paths $\OutA{+}{\Aconc}(\s)$ that are compatible with it along with a function $\ext_\B: \OutA{+}{\Aconc}(\s) \rightarrow \OutA{+}{\ATurnConc}(\sigma)$ ensuring that for all $\pi \in \OutA{+}{\Aconc}(\s)$, we have $\projec{V}{Q} \circ \ext_\B(\pi) = \pi$ and $\head(\ext_\B(\pi)) = \head(\pi)$.
	
	We set $\ext_\B(q_0) = q_0$. Now, assume that $\s$ is defined on paths of length at most $i-1$ and $\ext_\B$ on paths of length at most $i$ for some $i \geq 1$%(for $i = 1$, $\s$ is not defined anywhere)
	. Let $\pi \in \OutA{+}{\Aconc}(\s)$ such that $|\pi| = i$. Let us define $\s(\pi)$. Let $q = \head(\pi) = \head(\ext_\B(\pi)) \in Q$. Consider the function $\rch_\pi: A \rightarrow Q$ such that $\rch_\pi(a) = \sigma(\ext_\B(\pi) \cdot (q,\delta(q,a,B)))$, it associates to each action of Player $\A$ the state seen after the reaction of Player $\B$ in the turn-based arena $\ATurnConc$ if he follows the strategy $\sigma$. %set $Q_q = \{ \sigma(\ext_\B(\pi) \cdot (q,\delta(q,a,B))) \mid a \in A \} \subseteq Q$ of states reachable in two steps from $q$ in $\ATurnConc$ if Player $\B$ follows the strategy $\sigma$ and
	Now, consider the local interaction $\formNF_{q}$. We have $\reachStrat{\A}(\formNF_q,\delta(q,A,B) \setminus \rch_\pi[A]) = \emptyset$ since, for all $a \in A$, there exists $b \in B$ such that $\delta(q,a,b) = \rch_\pi(a) \in \rch_\pi[A]$. Therefore, since $\formNF_{q}$ is determined %(as the whole concurrent game $\Aconc$ is locally determined) 
	and by Proposition~\ref{prop:winning_set_determined}, we have $\reachStrat{\B}(\formNF_q,\rch_\pi[A]) \neq \emptyset$. Then, we set $\s(\pi) = \min_{<_B} \reachStrat{\B}(\formNF_q,\rch_\pi[A])$. 
	
	Now, assume that $\s$ is defined on paths of length at most $i$. Let $\pi  = \pi' \cdot q \in \OutA{+}{\Aconc}(\s)$ so that $|\pi| = i+1$. We define $\ext_\B(\pi)$. Let $q' = \head(\pi') \in Q$. By definition, we have $q \in \delta(q',A,\s(\pi'))$. Thus, by choice of $\s(\pi')$, we have $q \in \rch_{\pi'}[A]$. %Hence, we have $A_{q',q} := \{ a \in A \mid q = \sigma(\ext_\B(\pi') \cdot (q',\delta(q',a,B))) \} \neq \emptyset$. 
	We set $\ext_\B(\pi) = \ext_\B(\pi') \cdot (q',\delta(q',a,B)) \cdot q$ where $a = \min_{<_A} \rch_{\pi'}^{-1}[q]$. Note that $\ext_\B(\pi) \in  \OutA{+}{\ATurnConc}(\sigma)$ by definition of $\rch_{\pi'}$. Moreover, we have $\projec{V}{Q}(\ext_\B(\pi)) = \projec{V}{Q}(\ext_\B(\pi')) \cdot q = \pi' \cdot q = \pi$ and $\head(\ext_\B(\pi)) = q = \head(\pi)$.
	
	If we now consider an infinite path $\pi \in \OutA{\omega}{\Aconc}(\s)$, it follows that the infinite paths $\pi' \in \OutA{\omega}{\ATurnConc}(\sigma)$ with $\{ \ext_\B(\pi_{\leq i}) \mid i \geq 0 \}$ as prefixes ensures: $\pi' \in \OutA{\omega}{\ATurnConc}(\sigma)$ and $\projec{V}{Q}(\pi') = \pi$. That is, $\pi \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
\end{proof}
\begin{proof}
	The strategy $\s \in \SetStrat{\Aconc}{\B}$ is inductively defined on the set of paths $\OutA{+}{\Aconc}(\s)$ that are compatible with it. Note that if the strategy $\s$ is partially defined on paths of length up to $i-1$ for some $i \geq 1$, then we can consider paths compatible with $\s$ of length up to $i$. The strategy $\s$ is arbitrarily defined on paths that are not in $\OutA{+}{\Aconc}(\s)$. It is also defined along with a function $\ext_\B: \OutA{+}{\Aconc}(\s) \rightarrow \OutA{+}{\ATurnConc}(\sigma)$ ensuring that for all $\pi \in \OutA{+}{\Aconc}(\s)$, we have $\projec{V}{Q} \circ \ext_\B(\pi) = \pi$ and $\head(\ext_\B(\pi)) = \head(\pi)$.
	
	%We set $\ext_\B(q_0) = q_0$. Now, assume that $\s$ is defined on paths of 
	%length at most $i-1$ and $\ext_\B$ on paths of length at most $i$ for some 
	%$i \geq 1$ (for $i = 1$, $\s$ is not defined anywhere). Let $\pi \in 
	%\OutA{+}{\Aconc}(\s)$ such that $|\pi| = i$. Let us define $\s(\pi)$. Let 
	%$q = \head(\pi) = \head(\ext_\B(\pi)) \in Q$. Consider the set $Q_q = \{ 
	%\sigma(\ext_\B(\pi) \cdot (q,\delta(q,a,B))) \mid a \in A \} \subseteq Q$ 
	%of states reachable in two steps from $q$ in the turn-based game 
	%$\ATurnConc$ if Player $\B$ follows the strategy $\sigma$. Now consider 
	%the 
	%local interaction $\formNF_{q}$. We have 
	%$\reachStrat{\A}(\formNF_q,\delta(q,A,B) \setminus Q_q) = \emptyset$ 
	%since, 
	%for all $a \in A$, there is an action $b \in B$ for Player $\B$ such that 
	%$\delta(q,a,b) \in Q_q$. Therefore, since $\formNF_{q}$ is determined (as 
	%the whole concurrent game $\Aconc$ is locally determined) and by 
	%Proposition~\ref{prop:winning_set_determined}, we have 
	%$\reachStrat{\B}(\formNF_q,Q_q) \neq \emptyset$. Then, we set $\s(\pi) = 
	%\min_{<_B} \reachStrat{\B}(\formNF_q,Q_q)$. 
	
		We set $\ext_\B(q_0) = q_0$. Now, assume that $\s$ is defined on paths 
		of length at most $i-1$ and $\ext_\B$ on paths of length at most $i$ 
		for some $i \geq 1$%(for $i = 1$, $\s$ is not defined anywhere)
	. Let $\pi \in \OutA{+}{\Aconc}(\s)$ such that $|\pi| = i$. Let us define 
	$\s(\pi)$. Let $q = \head(\pi) = \head(\ext_\B(\pi)) \in Q$. Consider the 
	function $\rch_\pi: A \rightarrow Q$ such that $\rch_\pi(a) = 
	\sigma(\ext_\B(\pi) \cdot (q,\delta(q,a,B)))$, it associates to each action 
	of Player $\A$ the state seen after the reaction of Player $\B$ in the 
	turn-based arena $\ATurnConc$ if he follows the strategy $\sigma$. %set 
	%$Q_q = \{ \sigma(\ext_\B(\pi) \cdot (q,\delta(q,a,B))) \mid a \in A \} 
	%\subseteq Q$ of states reachable in two steps from $q$ in $\ATurnConc$ if 
	%Player $\B$ follows the strategy $\sigma$ and
	Now, consider the local interaction $\formNF_{q}$. We have 
	$\reachStrat{\A}(\formNF_q,\delta(q,A,B) \setminus \rch_\pi[A]) = 
	\emptyset$ since, for all $a \in A$, there exists $b \in B$ such that 
	$\delta(q,a,b) = \rch_\pi(a) \in \rch_\pi[A]$. Therefore, since 
	$\formNF_{q}$ is determined %(as the whole concurrent game $\Aconc$ is 
	%locally determined) 
	and by Proposition~\ref{prop:winning_set_determined}, we have 
	$\reachStrat{\B}(\formNF_q,\rch_\pi[A]) \neq \emptyset$. Then, we set 
	$\s(\pi) = \min_{<_B} \reachStrat{\B}(\formNF_q,\rch_\pi[A])$. 
	
	Let us now assume that $\s$ is defined on paths of length at most $i$. Let 
	$\pi  = \pi' \cdot q \in \OutA{+}{\Aconc}(\s)$ so that $|\pi| = i+1$. Let 
	us define $\ext_\B(\pi)$. Let $q' = \head(\pi') \in Q$. By definition, we 
	have $q \in \delta(q',A,\s(\pi'))$. Thus, 
	by choice of $\s(\pi')$, we have $q \in \rch_{\pi'}[A]$. %Hence, we have 
	%$A_{q',q} := \{ a \in A \mid q = \sigma(\ext_\B(\pi') \cdot 
	%(q',\delta(q',a,B))) \} \neq \emptyset$. 
	We set $\ext_\B(\pi) = \ext_\B(\pi') \cdot (q',\delta(q',a,B)) \cdot q$ 
	where $a = \min_{<_A} \rch_{\pi'}^{-1}[q]$. Note that $\ext_\B(\pi) \in  
	\OutA{+}{\ATurnConc}(\sigma)$ by definition of $\rch_{\pi'}$. Moreover, we 
	have $\projec{V}{Q}(\ext_\B(\pi)) = \projec{V}{Q}(\ext_\B(\pi')) \cdot q = 
	\pi' \cdot q = \pi$ and $\head(\ext_\B(\pi)) = q = \head(\pi)$.
	
	If we now consider an infinite path $\pi \in \OutA{\omega}{\Aconc}(\s)$, it follows that the infinite paths $\pi' \in \OutA{\omega}{\ATurnConc}(\sigma)$ with $\{ \ext_\B(\pi_{\leq i}) \mid i \geq 0 \}$ as prefixes ensures: $\pi' \in \OutA{\omega}{\ATurnConc}(\sigma)$ and $\projec{V}{Q}(\pi') = \pi$. That is, $\pi \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
\end{proof}

From the lemmas we have proved in this section, results the following theorem:
\begin{theorem}
	For all $W \subseteq Q^\omega$, the two-player concurrent graph game $\Games{\Aconc}{W}$ is determined if and only if its sequential version $\Games{\ATurnConc}{W^\Aconc}$ is and the same player has a winning strategy in both games.
	\label{thm:determinacy_equivalence}
\end{theorem}
\begin{proof}
	This comes from Lemmas~\ref{lem:inclusion_outcome_win},~\ref{lem:conc_to_turn},~\ref{lem:turn_to_conc_A} and~\ref{lem:turn_to_conc_B}.
\end{proof}

\bbcomment{The following seems too long}
\textbf{Application: Borel determinacy}
Let us apply Theorem~\ref{thm:determinacy_equivalence} to prove the Borel determinacy of locally determined concurrent games.
\begin{definition}
	For a non-empty set $D$ and $\pi \in D^*$, the \emph{cylinder} generated by $\pi$ is the set $\cyl(\pi) = \{ \pi \cdot \pi' \mid \pi' \in D^\omega \}$. Then, we call \emph{open sets} of $D^\omega$ arbitrary union of cylinders generated by finite sequence of elements of $D$. 
	
	The \emph{Borel set} on $D$ is the smallest collection of subsets $\Borel(D) \subseteq \partS(D^\omega)$ of $D^\omega$ such that all open sets of $D^\omega$ are in $\Borel(D)$, for all $B \in \Borel(D)$, $D^\omega \setminus B \in \Borel(D)$ and for all $(B_i)_{i \in \Nat} \in (\Borel(D))^{\Nat}$, we have $\bigcup_{i \in \Nat} B_i \in \Borel(D)$.
\end{definition}

We have the following result with Borel winning sets:
\begin{theorem}[Martin~\cite{martin1975borel,martin1985purely,martin1998determinacy}]
	Consider a turn-based graph arena $\Aturn = \AcoloredTurn$. For all Borel winning set $W \in \Borel(V)$, then the game $\Games{\Aturn}{W}$ is determined.
	\label{thm:turn_based_borel_determined}
\end{theorem}

We want to apply this theorem (along with Theorem~\ref{thm:determinacy_equivalence}) to prove that (locally determined) concurrent games with a Borel winning set are determined. To do so, we first have to prove that the transformation of the winning set preserves the "Borelness" of the set. We state a useful (and classical, see for instance \cite{moschovakis2009descriptive}) property on stability of Borel sets, then the lemma of interest for us follows.

\begin{proposition}
	Consider two arbitrary non-empty sets $D$ and $E$ and a function $\fex: \starom{D} \rightarrow \starom{E}$ such that, for all open set $E' \subseteq E$, we have $\fex^{-1}[E'] \in \Borel(D)$ ($\fex$ said to be continuous). Then, for all $B \in \Borel(E)$, we have $\fex^{-1}[B] \in \Borel(D)$.
	\label{prop:borel_stable_continuous}
\end{proposition}
\begin{lemma}
	Consider a concurrent graph arena $\Aconc = \AcoloredConc$. Then, for all $W \in \Borel(Q)$, we have $(\projec{V}{Q})^{-1}[W] \in \Borel(V)$ %where $V = Q \uplus Q \times A$
	.
	\label{lem:transfo_preserve_borel}
\end{lemma}
\begin{proof}
	It is quite straightforward to show that the function $\projec{V}{Q}: \starom{V} \rightarrow \starom{Q}$ is continuous. The lemma follows, by Property~\ref{prop:borel_stable_continuous}.
\end{proof}

We deduce the following corollary.
\begin{corollary}
	Consider a concurrent graph arena $\Aconc = \AcoloredConc$ that is locally determined. This arena is determined for $\Borel(Q)% \subseteq \partS(Q^\omega)
	$.
	\label{coro:conc_borel_determined}
\end{corollary}
\begin{proof}
	Consider a two-player concurrent graph game $\Games{\Aconc}{W}$ where $W \in \Borel(Q)$. By Theorem~\ref{thm:turn_based_borel_determined}, its sequential version $\Games{\ATurnConc}{W^\Aconc}$ is determined since, by Lemma~\ref{lem:transfo_preserve_borel}, the winning set $W^\Aconc$ is Borel. Hence, by Theorem~\ref{thm:determinacy_equivalence}, the concurrent game $\Games{\Aconc}{W}$ is determined.
\end{proof}

In turn, we get the following theorem:
\begin{theorem}
	Consider a set of game forms $\mathcal{I}$, and a set of colors $K$. Then the following assertions are equivalent:
	\begin{itemize}
		\item[1.] $\mathcal{I} \subseteq \allDet$; 
		\item[2.] For all Borel set $W \subseteq K^\omega$, all concurrent games built on $\mathcal{I}$ are determined for $W$;
		\item[2'.] There exists a Borel set $\emptyset \subsetneq W \subsetneq K^\omega$ such that all concurrent games  built on $\mathcal{I}$ is determined for $W$;
	\end{itemize}
\end{theorem}
\begin{proof}
	Implication $(1) \Rightarrow (2)$ comes from Corollary~\ref{coro:conc_borel_determined}, implication $(2) \Rightarrow (2')$ is straightforward and implication $(2') \Rightarrow (1)$ is given by Theorem~\ref{thm:locel_det_necessary_arbitrary_winning}.
\end{proof}


==> Tex/Memory.tex <==
The results we have proved in the previous section do not deal with the amount of memory required to implement a strategy. Indeed, we considered arbitrary strategies regardless of how they could be implemented. However, some kinds of objectives only require finite-memory strategies to be played optimally, or even only positional strategies. In 2005, the authors of \cite{DBLP:conf/concur/GimbertZ05} proved an equivalence between the shape of the winning set and the fact that positional strategies suffice to solve them. Similarly, in the recent paper \cite{DBLP:conf/concur/Bouyer0ORV20}, the authors generalized that result by establishing an equivalence relating  the shape of the winning set and the fact that strategies with a given memory skeleton are enough to play optimally. In the following, we establish that finite memory strategies can be translated into a concurrent game from its sequential version by using the same amount of memory and we prove that if a winning set ensures the conditions specified in \cite{DBLP:conf/concur/GimbertZ05} or \cite{DBLP:conf/concur/Bouyer0ORV20}, then its translation in the sequential version also does. \bbcomment{This should be rephrased}

\subsection{Finite memory strategies}
Let us define what finite memory strategies are. First, we recall the notion of memory skeleton that was introduced in \cite{DBLP:conf/concur/Bouyer0ORV20}.

\begin{definition}
	Consider a set of colors $\colSet$. A \emph{memory skeleton} on $\colSet$ is a triple $\langle M,m_{init},\mu \rangle$, where $M$ is a non-empty finite set (the memory), $m_{init} \in M$ is the initial state of the memory and $\mu: M \times \colSet \rightarrow M$ is the update function. A \emph{choice function} with memory $M$ is a function $\lambda: M \times D \rightarrow T$ for two non-empty sets $D$ and $T$. 
\end{definition}

We can now see how a memory skeleton and a choice function implement a strategy.
\begin{definition}
	Consider a colored arena $\langle \mathcal{G},\colSet,\colFunc \rangle$ (whether it is concurrent or turn-based) played on a set of states $D$, a player $\kappa \in \{ \A,\B \}$ who has to choose an element in $T$ when the current state of the game is in %a set 
	$D_\kappa \subseteq D$ (note that in a concurrent game, $D = D_\kappa$). Then, a memory skeleton $\langle M,m_{init},\mu \rangle$ on $\colSet$ and a choice function $\lambda: M \times D_\kappa \rightarrow T$ implement a strategy $\s_\kappa: D^* \cdot D_\kappa \rightarrow T$ such that $\s_\kappa(\rho) = \lambda(\extendFunc{\mu}(m_{init},\extendFunc{\colFunc}(\rho)),\head(\rho)) \in T$ for all $\rho \in D^* \cdot D_\kappa$.
	
	A strategy $\s$ is said to be \emph{finite memory} if there exists a memory skeleton $\langle M,m_{init},\mu \rangle$, where $M$ is finite, and a choice function $\lambda$ implementing $\s$. If $M$ is reduced to a singleton, $\s$ is said to be \emph{positional}. The amount of memory used to implement the strategy $\s$ is $|M|$.
\end{definition}

\begin{definition}
	A game %(whether it is concurrent or turn-based) 
	is said to be finite-memory (resp. positionally) determined if it is determined and winning strategies can be found among finite-memory (resp. positional) strategies.
\end{definition}

\subsection{Translating finite-memory strategies}
Let us now examine how we can translate finite-memory strategies from one arena to another. Let us first introduce two functions translating the memory update function. Informally, for $\colSetSeq = \colSet \uplus \{ k_\Aconc \}$, if we consider a memory update function $\mu$ in the concurrent game, the new memory update function $\trT(\mu)$ consists mimicking $\mu$ when a color in $\colSet$ is seen, whereas the memory is not changed if $k_\Aconc $ is seen. Reciprocally, from a memory update function $\mu$ in the turn-based game, when a color $k$ in $\colSet$ is seen, the new memory update function $\trC(\mu)$ consist of updating the memory once as if $k_\Aconc$ were seen and only then updating the memory with the color $k$.
\begin{definition}
	Let $\colSet$ be a set of colors and $\Aconc = \AcoloredConc$ be a concurrent arena, and $M$ be a non-empty set. For $\mu: M \times \colSet \rightarrow M$, we denote by $\trT(\mu) : M \times \colSetSeq \rightarrow M$ such that $\trT(\mu)(m,k) = \mu(m,k)$ and $\trT(\mu)(m,k_\Aconc) = m$ for all $m \in M$ and $k \in K$. 
	
	For $\mu: M \times \colSetSeq \rightarrow M$, we denote by $\trC(\mu) : M \times \colSet \rightarrow M$ such that $\trC(\mu)(m,k) = \mu(\mu(m,k_\Aconc),k)$ for all $m \in M$ and $k \in K$.
\end{definition}

We consider the simpler case of translation of strategies from a concurrent arena into its sequential version.
\begin{lemma}
	Let $\Aconc = \AcoloredConc$ be a concurrent arena and consider a player $\kappa \in \{ \A,\B \}$. Let $\s \in \SetStrat{\Aconc}{\kappa}$  be a strategy for Player $\kappa$ in the concurrent arena $\Aconc$ implemented by a memory skeleton $\langle M,m_{init},\mu \rangle$ on $\colSetSeq$ and a choice function $\lambda: M \times Q \rightarrow C$ where $C$ is the set of actions for Player $\kappa$. 
	
	Then, there exists a strategy $\sigma \in \SetStrat{\ATurnConc}{\kappa}$ for Player $\kappa$ in the sequential version $\ATurnConc$ implemented by 
	the memory skeleton $\langle M,m_{init},\trT(\mu) \rangle$ on $\colSet$ and a choice function $\lambda^\Aconc: M \times Q \rightarrow C$ where $C$ is the set of actions available for Player $\kappa$ ensuring: $\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)] \subseteq \OutA{\omega}{\Aconc}(\s)$.
	\label{lem:conc_to_turn_memory}
\end{lemma}
\begin{proof}
	Consider the case of Player $\A$. Let %$\mu^\Aconc: M \times \colSetSeq \rightarrow M$ be such that $\mu^\Aconc(m,k) = \mu(m,k)$ if $k \in \colSet$ and $\mu^\Aconc(m,k) = m$ otherwise and 
	$\lambda^\Aconc  = \transSeq \circ (\projTwo,\lambda) : M \times V_\A \rightarrow V$. It is straightforward to check that the strategy $\sigma \in \SetStrat{\ATurnConc}{\kappa}$ for Player $\kappa$ in the sequential version $\ATurnConc$ implemented by the memory skeleton $\langle M,m_0,\trT(\mu) \rangle$ and the choice function $\lambda^\Aconc$ is in fact equal to the strategy defined in Lemma~\ref{lem:conc_to_turn}. The case of Player $\B$ is analogous.
\end{proof}

Consider now how we can translate strategies into a concurrent arena from its sequential version while preserving an inclusion defined in Lemma~\ref{lem:inclusion_outcome_win}. We have the following lemma:
\begin{lemma}
	Let $\Aconc = \AcoloredConc$ be a concurrent arena and consider a player $\kappa \in \{ \A,\B \}$. Let $\sigma \in \SetStrat{\ATurnConc}{\kappa}$ be a strategy for Player $\kappa$ in the sequential version $\ATurnConc$ implemented by a memory skeleton $\langle M,m_{init},\mu \rangle$ on $\colSetSeq$ and a choice function $\lambda: M \times V_\kappa \rightarrow V$. 
	
	Then, there exists a strategy $\s \in \SetStrat{\Aconc}{\kappa}$ for Player $\kappa$ in the concurrent arena $\Aconc$ implemented by 
	the memory skeleton $\langle M,m_{init},\trC(\mu) \rangle$ on $\colSet$ and 
	a choice function $\lambda': M \times Q \rightarrow C$ where $C$ is the set 
	of actions available for Player $\kappa$ ensuring: 
	$\OutA{\omega}{\Aconc}(\s) \subseteq 
	\projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
	\label{lem:turn_to_conc_memory}
\end{lemma}
\begin{proof}[Proof sketch in the case of Player $\A$]
	Let %$\mu': M \times \colSet \rightarrow M$ be such that $\mu'(m,k) = \mu(\mu(m,k_{\Aconc}),k)$ for all $m \in \colSet$ and $k \in \colSet$ and 
	$\lambda'(m,q) = a$ such that $\lambda(m,q) = (q,\delta(q,a,B))$ for all $m \in M$ and $q \in Q = V_\A$. % where $\projTwo: V_\B \rightarrow A$ is the projection function on the second element of a pair defined in the proof of Lemma~\ref{lem:turn_to_conc_A}.
	Consider the strategy $\s$ implemented by the memory skeleton $\langle 
	M,m_{init},\trC(\mu) \rangle$ and the choice function $\lambda'$. 
	
	Note that, for all $\pi \in \OutA{*}{\ATurnConc}(\sigma)$, we have $\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi)) = \extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\projec{V}{Q}(\pi)))$. Now, for $\pi' \in \OutA{\omega}{\Aconc}(\s)$, we define $\pi \in V^\omega$ by $\pi_{2i} = \pi'_i \in Q$ and $\pi_{2i+1} = (\pi'_i,\delta(\pi'_i,\s(\pi'_{\leq i}),B)) \in V_\B$ for all $i \geq 0$. We have $\pi' = \projec{V}{Q}(\pi)$. Let us show by induction that $\pi_{\leq i} \in \OutA{*}{\ATurnConc}(\sigma)$ for all $i \geq 0$. We have $\pi_0 = \pi'_0 = q_0 \in \OutA{*}{\ATurnConc}(\sigma)$. Assume that $\pi_{\leq 2i} \in \OutA{*}{\ATurnConc}(\sigma)$ for some $i \geq 0$. We have $\sigma(\pi_{\leq 2i}) = \lambda(\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i})),\pi_{2i}) = (\pi_{2i},\delta(\pi_{2i},s(\pi'_{\leq i}),B))$ by definition of $\lambda'$ and since 	$\s(\pi'_{\leq i}) = \lambda'(\extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\pi'_{\leq i})),\head(\pi'_{\leq i})) = \lambda'(\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i})),\pi_{2i})$. Overall, $\sigma(\pi_{\leq 2i}) = (\pi'_{i},\delta(\pi'_{i},s(\pi'_{\leq i}),B)) = \pi_{2i+1}$. Hence, we have $\pi_{\leq 2i+1} \in \OutA{*}{\ATurnConc}(\sigma)$. Furthermore, $\pi_{2i+2} = \pi'_{i+1} \in Q$ with $\pi'_{i+1} \in \delta(\pi'_i,\s(\pi'_{\leq i}),B)$, thus $(\pi_{2i+1},\pi_{2i+2}) \in E_\B$. It follows that $\pi_{\leq 2i+2} \in \OutA{*}{\ATurnConc}(\sigma)$. In fact, we have $\pi \in \OutA{\omega}{\ATurnConc}(\sigma)$ and $\pi' \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
	%	such that $\pi' = \projec{V}{Q}(\pi)$. Let $\pi_0 = q_0 = \pi'_0$. Now, assume that $\pi \in \OutA{*}{\ATurnConc}(\sigma)$ is defined up to index $2i$ for some $i \geq 0$ and that $\projec{V}{Q}(\pi_{\leq 2i}) = \pi'_{\leq i}$. We have $\s(\pi'_{\leq i}) = \lambda'(\extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\pi'_{\leq i})),\head(\pi'_{\leq i})) = \projTwo \circ \lambda(\extendFunc{\trC(\mu)}(m_{init},\projec{\colSetSeq}{\colSet} \circ \extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i})),\pi'_{2i})$
\end{proof}
\begin{proof}[Proof in the case of Player $\A$]
	For all $m \in M$ and $q \in Q = V_\A$, let %$\mu': M \times \colSet 
	%\rightarrow M$ be such that $\mu'(m,k) = \mu(\mu(m,k_{\Aconc}),k)$ for all 
	%$m \in \colSet$ and $k \in \colSet$ and 
	$\lambda'(m,q) = \min_{<_\A} \{ a \in A \mid (q,\delta(q,a,B)) = 
	\lambda(m,q) \} \neq \emptyset$ since $\lambda(m,q) \in V_\B$. % where 
	%$\projTwo: V_\B \rightarrow A$ is the projection function on the second 
	%element of a pair defined in the proof of Lemma~\ref{lem:turn_to_conc_A}.
	Consider the strategy $\s$ implemented by the memory skeleton $\langle 
	M,m_{init},\trC(\mu) \rangle$ and the choice function $\lambda'$. 
	
	First, note that, for all $\pi \in \OutA{*}{\ATurnConc}(\sigma)$, we have 
	$\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi)) = 
	\extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\projec{V}{Q}(\pi)))$ 
	by definition of $\trC(\mu)$ and since, for all $i \geq 0$, we have 
	$\pi_i \in Q$ if and only if $i$ is even.
	
	Now, for $\pi' \in \OutA{\omega}{\Aconc}(\s)$, we define $\pi \in V^\omega$ by $\pi_{2i} = \pi'_i \in Q$ and $\pi_{2i+1} = (\pi'_i,\delta(\pi'_i,\s(\pi'_{\leq i}),B)) \in V_\B$ for all $i \geq 0$. Note that we have $\pi' = \projec{V}{Q}(\pi)$. Let us show by induction that $\pi_{\leq i} \in \OutA{*}{\ATurnConc}(\sigma)$ for all $i \geq 0$. We have $\pi_0 = \pi'_0 = q_0 \in \OutA{*}{\ATurnConc}(\sigma)$. Assume that $\pi_{\leq 2i} \in \OutA{*}{\ATurnConc}(\sigma)$ for some $i \geq 0$. We have $\s(\pi'_{\leq i}) = \lambda'(\extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\pi'_{\leq i})),\head(\pi'_{\leq i})) = \lambda'(\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i})),\pi_{2i}) = a$ for $a \in A$ such that  $\lambda(\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i})),\pi_{2i}) = (\pi_{2i},\delta(\pi_{2i},a,B))$. That is, $\sigma(\pi_{\leq 2i}) = (\pi_{2i},\delta(\pi_{2i},s(\pi'_{\leq i}),B)) = (\pi'_{i},\delta(\pi'_{i},s(\pi'_{\leq i}),B)) = \pi_{2i+1}$. Hence, we have $\pi_{\leq 2i+1} \in \OutA{*}{\ATurnConc}(\sigma)$. Furthermore, we have $\pi_{2i+2} = \pi'_{i+1} \in Q$ with $\pi'_{i+1} \in \delta(\pi'_i,\s(\pi'_{\leq i}),B)$, that is $(\pi_{2i+1},\pi_{2i+2}) \in E_\B$. It follows that $\pi_{\leq 2i+2} \in \OutA{*}{\ATurnConc}(\sigma)$. Overall, we have $\pi \in \OutA{\omega}{\ATurnConc}(\sigma)$ and $\pi' \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
%	such that $\pi' = \projec{V}{Q}(\pi)$. Let $\pi_0 = q_0 = \pi'_0$. Now, assume that $\pi \in \OutA{*}{\ATurnConc}(\sigma)$ is defined up to index $2i$ for some $i \geq 0$ and that $\projec{V}{Q}(\pi_{\leq 2i}) = \pi'_{\leq i}$. We have $\s(\pi'_{\leq i}) = \lambda'(\extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\pi'_{\leq i})),\head(\pi'_{\leq i})) = \projTwo \circ \lambda(\extendFunc{\trC(\mu)}(m_{init},\projec{\colSetSeq}{\colSet} \circ \extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i})),\pi'_{2i})$
\end{proof}

The proof for Player $\B$ is analogous, with the additional use of the local determinacy hypothesis.
\begin{proof}[Proof sketch in the case of Player $\B$]
	%We consider the same update function $\mu': M \times \colSet \rightarrow M$ than for the case of Player $\A$: $\mu'(m,k) = \mu(\mu(m,k_{\Aconc}),k)$ for all $m \in \colSet$ and $k \in \colSet$. 
	For $m \in M$ and $q \in Q$, we define the function $\reach{m}{q}: A \rightarrow Q$ such that $\reach{m}{q}(a) = \lambda(\mu(m,k_\Aconc),(q,\delta(q,a,B))) \in Q$, which is anlogous to the function $\rch_\pi$ defined in the proof of Lemma~\ref{lem:turn_to_conc_B}. % that is the function $\reach{m}{q}$ associates to an action for Player $\A$ the next state reached in the turn-based game $\ATurnConc$ if Player $\B$ follows his strategy $\sigma$ from the state $q$ with $m \in M$ as the state of the memory. 
	Then, we can see that, for all $m \in M$, $q \in Q$, and for all action $a \in A$ for Player $\A$, there exists $b \in B$, such that $\delta(q,a,b) = \reach{m}{q}(a) \in \reach{m}{q}[A]$. Hence, in the local interaction $\formNF_q$, we have that $\reachStrat{\A}(\formNF_q,\delta(q,A,B) \setminus \reach{m}{q}[A]) = \emptyset$. By determinacy of the game form $\formNF_q$, we have that $\reachStrat{\B}(\formNF_q,\reach{m}{q}[A]) \neq \emptyset$. We define the function $\lambda': M \times Q \rightarrow B$ such that, for all $m \in M$ and $q \in Q$, we have $\lambda'(m,q) = \min_{<_B} \reachStrat{\B}(\formNF_q,\reach{m}{q}[A])$.
	
	Consider the strategy $\s$ implemented by the memory skeleton $\langle M,m_0,\trC(\mu) \rangle$ and the choice function $\lambda'$. Let $\pi' \in \OutA{\omega}{\Aconc}(\s)$. For all $i \geq 0$, we denote by $m_i \in M$ the state of the memory after having seen $\pi'_{\leq i}$: $m_i = \extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\pi'_{\leq i}))$. Then, for all $i \geq 0$, we have $\s(\pi'_{\leq i}) = \lambda'(m_i,\pi'_i)$ and $\pi'_{i+1} \in \reach{m_i}{\pi'_i}[A]$. Let us define $\pi \in V^\omega$ by $\pi_{2i} = \pi'_i \in Q$ and $\pi_{2i+1} = (\pi'_i,\delta(\pi'_i,a_i,B)) \in V_\B$ where $a_i = \min_{<_A} \inv{\reach{m_i}{\pi'_{i}}}[\{\pi'_{i+1}\}] \neq \emptyset$ for all $i \geq 0$. With this definition, we have $\projec{V}{Q}(\pi) = \pi'$. We show by induction that for all $i \geq 0$, we have $\pi_{\leq i} \in \OutA{*}{\ATurnConc}(\sigma)$. We have $\pi_0 = \pi'_0 = q_0 \in \OutA{*}{\ATurnConc}(\sigma)$. Now, assume that $\pi_{\leq 2i} \in \OutA{*}{\ATurnConc}(\sigma)$ for some $i \geq 0$. We have $\pi_{2i+1} = (\pi'_i,\delta(\pi'_i,a_i,B)) = (\pi_{2i},\delta(\pi_{2i},a_i,B))$ hence $\pi_{\leq 2i+1} \in \OutA{*}{\ATurnConc}(\sigma)$. Furthermore, we have $m_i = \extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\pi'_{\leq i})) = \extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i}))$%, because as in the case of Player $\A$ for all $\pi \in \OutA{*}{\ATurnConc}(\sigma)$, we have $\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi)) = \extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\projec{V}{Q}(\pi)))$
	. Hence, $\sigma(\pi_{\leq 2i+1}) = \lambda(\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i+1})),\pi_{2i+1}) = \lambda(\mu(m_i,k_\Aconc),(\pi_{2i},\delta(\pi_{2i},a_i,B))) = \reach{m_i}{\pi_{2i}}(a_i) = \reach{m_i}{\pi'_{i}}(a_i)$. Since $a_i \in \inv{\reach{m_i}{\pi'_{i}}}[\{\pi'_{i+1}\}]$, we have $\sigma(\pi_{\leq 2i+1}) = \pi'_{i+1} = \pi_{2i+2}$. Hence, $\pi_{\leq 2i+2} \in \OutA{*}{\ATurnConc}(\sigma)$. Overall, we have $\pi \in \OutA{\omega}{\ATurnConc}(\sigma)$ and $\pi' \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
\end{proof}

\begin{proof}[Proof in the case of Player $\B$]
	%We consider the same update function $\mu': M \times \colSet \rightarrow M$ than for the case of Player $\A$: $\mu'(m,k) = \mu(\mu(m,k_{\Aconc}),k)$ for all $m \in \colSet$ and $k \in \colSet$. 
	To define the choice function $\lambda': M \times Q \rightarrow B$, we first have to define an other function. For $m \in M$ and $q \in Q$, we define the function $\reach{m}{q}: A \rightarrow Q$ such that $\reach{m}{q}(a) = \lambda(\mu(m,k_\Aconc),(q,\delta(q,a,B))) \in Q$, that is the function $\reach{m}{q}$ associates to an action for Player $\A$ the next state reached in the turn-based game $\ATurnConc$ if Player $\B$ follows his strategy $\sigma$ from the state $q$ with $m \in M$ as the state of the memory. Then, we can see that, for all $m \in M$ and $q \in Q$, Player $\A$ cannot avoid the set $\reach{m}{q}[A]$ from $q$: that is, for all $a \in A$, there exists $b \in B$, such that $\delta(q,a,b) \in \reach{m}{q}[A]$. Hence, if we now consider the local interaction $\formNF_q$, we have that $\reachStrat{\A}(\formNF_q,\delta(q,A,B) \setminus \reach{m}{q}[A]) = \emptyset$. By determinacy of the game form $\formNF_q$, we have that $\reachStrat{\B}(\formNF_q,\reach{m}{q}[A]) \neq \emptyset$. We can now define the function $\lambda': M \times Q \rightarrow B$ such that, for all $m \in M$ and $q \in Q$, we have $\lambda'(m,q) = \min_{<_B} \reachStrat{\B}(\formNF_q,\reach{m}{q}[A])$.
	
	Now, consider the strategy $\s$ implemented by the memory skeleton $\langle M,m_0,\trC(\mu) \rangle$ and the choice function $\lambda'$. Let $\pi' \in \OutA{\omega}{\Aconc}(\s)$. For all $i \geq 0$, we denote by $m_i \in M$ the state of the memory after having seen $\pi'_{\leq i}$: $m_i = \extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\pi'_{\leq i}))$. Then, for all $i \geq 0$, we have $\s(\pi'_{\leq i}) = \lambda'(m_i,\pi'_i)$. It follows that, for all $i \geq 0$, we have $\pi'_{i+1} \in \reach{m_i}{\pi'_i}[A]$. Let us define $\pi \in V^\omega$ by $\pi_{2i} = \pi'_i \in Q$ and $\pi_{2i+1} = (\pi'_i,\delta(\pi'_i,a_i,B)) \in V_\B$ where $a_i = \min_{<_A} \inv{\reach{m_i}{\pi'_{i}}}[\{\pi'_{i+1}\}] \neq \emptyset$ for all $i \geq 0$. With this definition, we have $\projec{V}{Q}(\pi) = \pi'$. Let us show by induction that for all $i \geq 0$, we have $\pi_{\leq i} \in \OutA{*}{\ATurnConc}(\sigma)$. We have $\pi_0 = \pi'_0 = q_0 \in \OutA{*}{\ATurnConc}(\sigma)$. Now, let us assume that $\pi_{\leq 2i} \in \OutA{*}{\ATurnConc}(\sigma)$ for some $i \geq 0$. We have $\pi_{2i+1} = (\pi'_i,\delta(\pi'_i,a_i,B))$ hence $\pi_{\leq 2i+1} \in \OutA{*}{\ATurnConc}(\sigma)$ since $\pi'_i = \pi_{2i}$. Furthermore, we have $m_i = \extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\pi'_{\leq i})) = \extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i}))$, because as in the case of Player $\A$ for all $\pi \in \OutA{*}{\ATurnConc}(\sigma)$, we have $\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi)) = \extendFunc{\trC(\mu)}(m_{init},\extendFunc{\colFunc}(\projec{V}{Q}(\pi)))$. Hence, $\sigma(\pi_{\leq 2i+1}) = \lambda(\extendFunc{\mu}(m_{init},\extendFunc{\colFunc_\Aconc}(\pi_{\leq 2i+1})),\pi_{2i+1}) = \lambda(\mu(m_i,\colFunc_\Aconc(\pi_{2i},\pi_{2i+1})),(\pi_{2i},\delta(\pi'_i,a_i,B))) = \lambda(\mu(m_i,k_\Aconc),(\pi_{2i},\delta(\pi_{2i},a_i,B))) = \reach{m_i}{\pi_{2i}}(a_i) = \reach{m_i}{\pi'_{i}}(a_i)$. Since $a_i \in \inv{\reach{m_i}{\pi'_{i}}}[\{\pi'_{i+1}\}]$, we have $\sigma(\pi_{\leq 2i+1}) = \pi'_{i+1} = \pi_{2i+2}$. Hence, $\pi_{\leq 2i+2} \in \OutA{*}{\ATurnConc}(\sigma)$. Overall, we have $\pi \in \OutA{\omega}{\ATurnConc}(\sigma)$ and $\pi' \in \projec{V}{Q}[\OutA{\omega}{\ATurnConc}(\sigma)]$.
\end{proof}

From the lemmas we have proved in this section, results the following theorem:
\begin{theorem}
	For all $W \subseteq \colSet^\omega$, the concurrent game 
	$\Games{\Aconc}{W}$ is finite-memory determined with $k \in \Nat$ amount of 
	memory necessary if and only if its sequential version 
	$\Games{\ATurnConc}{W^\Aconc}$ is and the same player has a winning 
	strategy.
	\label{thm:determinacy_equivalence_memory}
\end{theorem}
\begin{proof}
	This comes from Lemmas~\ref{lem:inclusion_outcome_win},~\ref{lem:conc_to_turn_memory} and~\ref{lem:turn_to_conc_memory}.
\end{proof}

\subsection{Condition for finite-memory determinacy in concurrent games}

\subsubsection{Definitions from \cite{DBLP:conf/concur/Bouyer0ORV20}}
We recall here the condition for the existence of finite memory strategy in turn-based games established in \cite{DBLP:conf/concur/Bouyer0ORV20}. In the following, we will be considering a set of colors $\colSet$ and a concurrent arena $\Aconc = \AcoloredConc$.

First, in \cite{DBLP:conf/concur/Bouyer0ORV20}, the authors do not consider a winning set $W \subseteq \colSet^\omega$ but rather a preference relation $\preceq: \colSet^\omega \times \colSet^\omega$ for Player $\A$ and the antagonistic preference $\preceq^{-1}$ for Player $\B$. Hence, we need to translate a winning set into a %n equivalent
preference relation. For $W \subseteq \colSet^\omega$, we consider the preference relation $\preceq_W: \colSet^\omega \times \colSet^\omega$ defined by $\rho \prec_W \rho'$ for all $\rho \not \in W$ and $\rho' \in W$.

Furthermore, the authors do not consider winning strategies, but optimal ones. However, it has to be noted that a winning strategy with a winning set $W \subseteq \colSet^\omega$ is an optimal strategy with preference $\preceq_W$ whereas the converse does not hold: if a player has no winning strategy, every one of his strategy is optimal, whereas if a player has a winning strategy, optimal and winning strategies coincide.

Let us now focus more closely on the condition stated in 
\cite{DBLP:conf/concur/Bouyer0ORV20} for the existence of optimal finite-memory 
strategies. Consider a language $L \subseteq \colSet^*$. The language $[L] := 
\{ \rho \in \colSet^\omega \mid \forall n \in \Nat,\; \exists \pi \in L,\; 
\rho_{\leq n} \sqsubset \pi \}$ refers to the set of infinite words whose 
prefixes are also the prefixes of a word in $L$. Furthermore, the notation 
$\rec(\colSet)$ refers to the regular languages on a finite subset of 
$\colSet$. In addition, for a preference $\preceq \subseteq \colSet^\omega 
\times \colSet^\omega$, and two languages $L,L' \subseteq \colSet^\omega$, $L 
\preceq L'$ refers to $\forall \rho \in L,\; \exists \rho' \in L',\; \rho 
\preceq \rho'$ and $L \prec L'$ refers to $\exists \rho' \in L',\; \forall \rho 
\in L,\; \rho \prec \rho'$. Note that $L \prec L' \Leftrightarrow \lnot (L' 
\preceq L)$. Finally, for a memory skeleton $\langle M,m_{init},\mu \rangle$ on 
$\colSet$, and two states of the memory $m,m' \in M$, we denote 
$L^\mathcal{M}_{m,m'} := \{ \rho \in \colSet^* \mid 
\extendFunc{\mu}(m,\extendFunc{\colFunc}(\rho)) = m' \}$. Let us consider the 
definitions of $\mathcal{M}$-monotony and $\mathcal{M}$-selectivity from 
\cite{DBLP:conf/concur/Bouyer0ORV20}:

\begin{definition}
	Let $\mathcal{M} = \langle M,m_{init},\mu \rangle$ be a memory skeleton. A preferences $\preceq \subseteq \colSet^\omega \times \colSet^\omega$ is $\mathcal{M}$-monotone if, for all $m \in M$ and $L_1,L_2 \in \rec(\colSet)$: $(\exists \rho \in L^\mathcal{M}_{m_{init},m},\; [\rho \cdot L_1] \prec [\rho \cdot L_2]) \Rightarrow (\forall \rho' \in L^\mathcal{M}_{m_{init},m}, [\rho' \cdot L_1] \preceq [\rho' \cdot L_2])$.
\end{definition}

\begin{definition}
	Let $\mathcal{M} = \langle M,m_{init},\mu \rangle$ be a memory skeleton. A preferences $\preceq \subseteq \colSet^\omega \times \colSet^\omega$ is $\mathcal{M}$-selective if, for all $\rho \in \colSet^*,\; m = \extendFunc{\mu}(m_{init},\extendFunc{\colFunc}(\rho)) \in M$, for all $L_1,L_2 \in \rec(\colSet)$ such that $L_1,L_2 \subseteq L^\mathcal{M}_{m,m}$, for all $L_3 \in \rec(\colSet)$, $[\rho \cdot (L_1 \cup L_2)^* \cdot L_3] \preceq [\rho \cdot L_1^*] \cup [\rho \cdot L_2^*] \cup [\rho \cdot L_3]$.
\end{definition}

Then the authors proved the following result (Theorem 9 in \cite{DBLP:conf/concur/Bouyer0ORV20}):
\begin{theorem}
	Let $\preceq \subseteq \colSet^\omega \times \colSet^\omega$ be a preference relation and $\mathcal{M}$ be a memory skeleton. Then, both players have  finite-memory strategies implemented with memory skeleton $\mathcal{M}$ in all finite turn-based games if and only if $\preceq$ and $\preceq^{-1}$ are $\mathcal{M}$-monotone and $\mathcal{M}$-selective.
	\label{thm:turn_equiv_memory_winning}
\end{theorem}

Note that when $M$ is a singleton, this characterization coincide with the earlier one proved in \cite{DBLP:conf/concur/GimbertZ05}.

\subsubsection{Monotony and selectivity equivalence}
For a memory skeleton $\mathcal{M} = \langle M,m_{init},\mu \rangle$ on $\colSet$, we denote by $\mathcal{M}^\Aconc = \langle M,m_{init},\trT(\mu) \rangle$ the memory skeleton on $\colSetSeq$ (similar to the proof of Lemma~\ref{lem:conc_to_turn_memory}). We establish the following theorem:
\begin{theorem}
	 Let $W$ be a winning condition in the concurrent arena $\Aconc = \AcoloredConc$, $\langle \ATurnConc,W^\Aconc \rangle$ be the sequential version of the concurrent game $\langle \Aconc,W \rangle$, and let $\mathcal{M}$ be a memory skeleton on $\colSet$. Then, $\preceq_W \subseteq \colSet \times \colSet$ is $\mathcal{M}$-monotone and $\mathcal{M}$-selective if and only if $\preceq_{W^\Aconc} \subseteq \colSetSeq \times \colSetSeq$ is $\mathcal{M}^\Aconc$-monotone and $\mathcal{M}^\Aconc$-selective.
	 \label{thm:winning_condition_stability}
\end{theorem}
Before proving this theorem, we state and prove a few simpler lemmas. Recall 
that $W^\Aconc = \inv{\projec{\colSetSeq}{\colSet}}[W]$.
\begin{lemma}
	For all $L \subseteq \starom{\colSet}$, we have $L = \projec{\colSet_\Aconc}{\colSet}[\inv{\projec{\colSet_\Aconc}{\colSet}}[L]]$.
	\label{lem:projection_equality_surjectivity}
\end{lemma}
\begin{proof}
	This is straightforward, by surjectivity of the projection 
	$\projec{\colSet_\Aconc}{\colSet}: \starom{\colSetSeq} \rightarrow 
	\starom{\colSet}$.
\end{proof}

\begin{lemma}
	For all $L_1,L_2 \subseteq \starom{\colSetSeq}$, we have $\projec{\colSetSeq}{\colSet}[L_1 \cup L_2] = \projec{\colSetSeq}{\colSet}[L_1] \; \cup \; \projec{\colSetSeq}{\colSet}[L_2]$. Furthermore, if $L_1 \subseteq \colSetSeq^*$, $\projec{\colSetSeq}{\colSet}[L_1 \cdot L_2] = \projec{\colSetSeq}{\colSet}[L_1] \; \cdot \; \projec{\colSetSeq}{\colSet}[L_2]$, and $\projec{\colSetSeq}{\colSet}[L_1^*] = (\projec{\colSetSeq}{\colSet}[L_1])^*$.
	\label{lem:algebraic_properties_projection}
\end{lemma}
\begin{proof}
	This is straightforward, by definition of the function $\projec{\colSet_\Aconc}{\colSet}$.
\end{proof}

\begin{lemma}
	For $L \subseteq \colSetSeq^*$, we have $L \in \rec(\colSetSeq) \Rightarrow \projec{\colSet_\Aconc}{\colSet}[L] \in \rec(\colSet)$. For $L \subseteq \colSet^*$, we have $L \in \rec(\colSet) \Leftrightarrow \projec{\colSet_\Aconc}{\colSet}^{-1}[L] \in \rec(\colSetSeq)$ 
	\label{lem:rationnal_stability_projection}
\end{lemma}
\begin{proof}
	Assume that $L \in \rec(\colSetSeq)$. Then, we can modify a finite automaton recognizing $L$ with a finite alphabet of $\colSetSeq$ by replacing every transition where $k_\Aconc$ appears by an $\epsilon$-transition. Then, the obtained automaton is finite and recognizes the language $\projec{\colSet_\Aconc}{\colSet}[L]$.
	
	Furthermore, a finite automaton recognizing the language $L$ with a finite alphabet on $\colSet$ can be modified by adding self loops labeled by $k_\Aconc$ on every state. The obtained automaton is finite and recognizes the language $\projec{\colSet_\Aconc}{\colSet}^{-1}[L]$. Finally, if $\projec{\colSet_\Aconc}{\colSet}^{-1}[L] \in \rec(\colSetSeq)$, then, with Lemma~\ref{lem:projection_equality_surjectivity},  $\projec{\colSet_\Aconc}{\colSet}[\projec{\colSet_\Aconc}{\colSet}^{-1}[L]] = L \in \rec(\colSet)$.
\end{proof}

\begin{lemma}
	For all $m,m' \in M$, we have: $L^\mathcal{M}_{m,m'} = \projec{\colSet_\Aconc}{\colSet}[L^{\mathcal{M}^\Aconc}_{m,m'}]$.
	\label{lem:language_equality_projection}
\end{lemma}
\begin{proof}
	Let $\rho \in \colSetSeq^*$. By definition of $\trT(\mu)$, we have $\extendFunc{\trT(\mu)}(m,\extendFunc{\colFunc_\Aconc}(\rho)) = \extendFunc{\mu}(m,\extendFunc{\colFunc}(\projec{\colSet_\Aconc}{\colSet}(\rho)))$. Hence, $\rho \in L^{\mathcal{M}^\Aconc}_{m,m'} \Leftrightarrow \projec{\colSet_\Aconc}{\colSet}(\rho) \in L^\mathcal{M}_{m,m'}$.
\end{proof}

\begin{lemma}
	For all $N_1,N_2 \subseteq \colSet^\omega_\Aconc$, we have $N_1 \prec_{W^\Aconc} N_2 \Leftrightarrow \colSet^\omega \cap \projec{\colSet_\Aconc}{\colSet}[N_1] \prec_{W} \colSet^\omega \cap \projec{\colSet_\Aconc}{\colSet}[N_2]$.
	\label{lem:inequality_stability_projection}
\end{lemma}
\begin{proof}
	By definition of the preference relation $\prec_{W^\Aconc}$, we have $N_1 \prec_{W^\Aconc} N_2 \Leftrightarrow N_1 \cap W^\Aconc = \emptyset \wedge N_2 \cap W^\Aconc \neq \emptyset \Leftrightarrow N_1 \cap \projec{\colSetSeq}{\colSet}^{-1}[W] = \emptyset \wedge N_2 \cap \projec{\colSetSeq}{\colSet}^{-1}[W] \neq \emptyset \Leftrightarrow (\colSet^\omega \cap \projec{\colSetSeq}{\colSet}[N_1]) \cap W = \emptyset \wedge (\colSet^\omega \cap \projec{\colSetSeq}{\colSet}[N_2]) \cap W \neq \emptyset \Leftrightarrow (\colSet^\omega \cap \projec{\colSetSeq}{\colSet}[N_1]) \prec_{W} (\colSet^\omega \cap \projec{\colSetSeq}{\colSet}[N_2])$.
\end{proof}

\begin{lemma}
	For all $L \in \rec(\colSetSeq)$, we have $\colSet^\omega \cap \projec{\colSet_\Aconc}{\colSet}[\; [L] \;] = [\projec{\colSet_\Aconc}{\colSet}[L]]$.
	\label{lem:projection_infinite_language}
\end{lemma}
\begin{proof}
	Let $L \subseteq \colSet^{*}_\Aconc$. Let us prove $\colSet^\omega \cap \projec{\colSet_\Aconc}{\colSet}[\; [L] \;] \subseteq [\projec{\colSet_\Aconc}{\colSet}[L]]$. Let $\rho = \projec{\colSet_\Aconc}{\colSet}(\rho') \in \colSet^\omega \cap \projec{\colSet_\Aconc}{\colSet}[\; [L] \;]$ with $\rho' \in [L]$. Let $\varphi: \Nat \rightarrow \Nat$ such that $\rho_{\leq n} = \projec{\colSet_\Aconc}{\colSet}(\rho'_{\leq \varphi(n)})$ for all $n \geq 0$. Then, for all $n \geq 0$, there exists $l^n \in L$ such that $\rho'_{\leq n} \sqsubseteq l^n$. It follows that, for all $n \geq 0$, we have $\rho_{\leq n} = \projec{\colSet_\Aconc}{\colSet}(\rho'_{\varphi(n)}) \sqsubseteq \projec{\colSet_\Aconc}{\colSet}(l^{\varphi(n)}) \in \projec{\colSet_\Aconc}{\colSet}[L]$. Hence, $\rho \in [\; \projec{\colSet_\Aconc}{\colSet}[L] \; ]$.
	
	Let us now prove that $\projec{\colSet_\Aconc}{\colSet}[\; [L] \;] \supseteq [\projec{\colSet_\Aconc}{\colSet}[L]]$. Since $L \in \rec(\colSetSeq)$, there exists a finite automaton $\mathcal{A}$ recognizing $L$. Let us denote by $i$ the number of states of $\mathcal{A}$. Let $\rho \in [\projec{\colSet_\Aconc}{\colSet}[L]]$. Then, for all $n \in \Nat$, there exists $u^n \in \projec{\colSet_\Aconc}{\colSet}[L]$ such that $\rho_{\leq n} \sqsubseteq u^n = \projec{\colSet_\Aconc}{\colSet}(v^n)$ for some $v^n \in L$ that we choose so that there is no sequence in $(k_\Aconc)^*$ longer than $i$ appearing in $v^n$. For all $n \geq 0$, let $l^n \sqsubseteq v^n$ be a prefix of $v_n$ such that $\rho_{\leq n} = \projec{\colSet_\Aconc}{\colSet}(l^n)$. In turn, with our choice for $v^n$, we have that for all $k \leq |l^n|-1$, $|l^n_{\leq k}| \leq i \times (|\projec{\colSetSeq}{\colSet}(l^n_{\leq k})| + 1)$. Then, the set of prefixes $\{ l^n \mid n \geq 0 \}$ is infinite, with finitely many colors, since $L \in \rec(\colSetSeq)$. Hence, by Koenig's lemma \bbcomment{(ref ?)}, we have $[ \{ l^n \mid n \geq 0 \} ] \neq \emptyset$. Let $l \in [ \{ l^n \mid n \geq 0 \} ]$. Then, for all $n \geq 0$, we have $l_{\leq n} \sqsubseteq l^k \sqsubseteq v^k \in L$ for some $k \in \Nat$. Hence, $l \in [L]$. Let us now show that $\projec{\colSetSeq}{\colSet}(l) \in \colSet^\omega$. To do so, we prove that $|\projec{\colSetSeq}{\colSet}(l_{\leq n})| \xrightarrow[n \to \infty]{} \infty$. Let $N \geq 0$. We set $n_0 = (N + 1) \cdot i \in \Nat$. Let $n \geq n_0$. There exists $n' \in \Nat$ such that $l_{\leq n} \sqsubseteq l^{n'}$. Hence, we have $|\projec{\colSetSeq}{\colSet}(l_{\leq n})| = |\projec{\colSetSeq}{\colSet}(l^{n'}_{\leq n})| \geq |l^{n'}_{\leq n}|/i - 1 = (n+1)/i - 1 \geq N$ since $n \geq (N+1) \cdot i$. It follows that $\projec{\colSetSeq}{\colSet}(l) \in \colSet^\omega$. Then, for all $n \in \Nat$, we have $\projec{\colSet_\Aconc}{\colSet}(l)_{\leq n} \sqsubseteq \projec{\colSet_\Aconc}{\colSet}(l^k_{\leq n}) \sqsubseteq \rho_{\leq k} \sqsubseteq \rho$ for some $k \in \Nat$. It follows that $\rho = \projec{\colSet_\Aconc}{\colSet}(l)$.
\end{proof}

We can now proceed to the proof of Theorem~\ref{thm:winning_condition_stability}.
\begin{proof}
	We prove the equivalence of monotony. The case of selectivity is similar. In the following, $\projec{\colSet_\Aconc}{\colSet}$ will be abbreviated $\proj$. Let $m \in M$, $L_1,L_2 \in \rec(\colSetSeq)$, $L'_1,L'_2 \in \rec(\colSet)$, and $\rho \in L^{\mathcal{M}_\Aconc}_{m_{init},m}$. Assume that $L'_1 = \proj(L_1)$ and $L'_2 = \proj(L_2)$. In that case:
	\begin{align*}
	[\rho \cdot L_1] \prec_{W^\Aconc}  [\rho \cdot L_2] &\Leftrightarrow \colSet^\omega \cap \proj[ \; [\rho \cdot L_1] \; ] \prec_{W} \colSet^\omega \cap \proj[ \; [\rho \cdot L_2] \; ] & \text{ by Lemma~\ref{lem:inequality_stability_projection}} \\
	&\Leftrightarrow [ \; \proj[\rho \cdot L_1] \; ] \prec_{W} [ \; \proj[\rho \cdot L_2] \; ] & \text{by Lemma~\ref{lem:projection_infinite_language}}\\
	&\Leftrightarrow [ \; \proj(\rho) \cdot L'_1 \; ] \prec_{W} [ \; \proj(\rho) \cdot L'_2 \; ] & \text{by Lemma~\ref{lem:algebraic_properties_projection}}
	\end{align*}
	%with $\projec{\colSet_\Aconc}{\colSet}[L_1],\projec{\colSet_\Aconc}{\colSet}[L_2] \in \rec(\colSet)$ by Lemma~\ref{lem:rationnal_stability_projection}. 
	The two following equivalences are then given by Lemma~\ref{lem:language_equality_projection}:
	\begin{displaymath}
		(\exists \rho \in L^{\mathcal{M}_\Aconc}_{m_{init},m},\; [\rho \cdot L_1] \prec_{W^\Aconc} [\rho \cdot L_2]) \Leftrightarrow (\exists \rho' \in L^\mathcal{M}_{m_{init},m},\; [\rho' \cdot L'_1] \prec_W [\rho' \cdot L'_2])
	\end{displaymath}
	Similarly, with a universal quantifier:
	\begin{displaymath}
	(\forall \rho \in L^{\mathcal{M}_\Aconc}_{m_{init},m},\; [\rho \cdot L_1] \preceq_{W^\Aconc} [\rho \cdot L_2]) \Leftrightarrow (\forall \rho' \in L^\mathcal{M}_{m_{init},m},\; [\rho' \cdot L'_1] \preceq_W [\rho' \cdot L'_2])
	\end{displaymath}
	By Lemma~\ref{lem:rationnal_stability_projection}, this holds for two arbitrary sets $L_1,L_2 \in \rec(\colSetSeq)$ and $\proj(L_1),\proj(L_2) \in \rec(\colSet)$. It also does with two arbitrary sets $L'_1,L'_2 \in \rec(\colSet)$ and $\proj^{-1}(L'_1),\proj^{-1}(L'_2) \in \rec(\colSetSeq)$, by Lemma~\ref{lem:projection_equality_surjectivity}. It follows that $\preceq_W$ is $\mathcal{M}$-monotone if and only if $\preceq_{W^\Aconc}$ is $\mathcal{M}^\Aconc$-monotone.	
\end{proof}


We can now state and prove the following theorem:
\begin{theorem}
	Let $W \subseteq \colSet^\omega$ be a winning set and $\mathcal{M}$ be a memory skeleton. Then, winning strategies for both players can be found among finite-memory strategies implemented with memory skeleton $\mathcal{M}$ in all finite locally determined concurrent games if and only if $\preceq_W$ and $\preceq_W^{-1}$ are $\mathcal{M}$-monotone and $\mathcal{M}$-selective.
	\label{thm:conc_equiv_memory_winning}
\end{theorem}
\begin{proof}
	If either $\preceq_W$ or $\preceq_W^{-1}$ is not $\mathcal{M}$-monotone and $\mathcal{M}$-selective, then Theorem~\ref{thm:turn_equiv_memory_winning} gives us an example of a finite turn-based game, which is a special case of finite locally determined concurrent games, where the players do not have optimal strategies implemented with memory skeleton $\mathcal{M}$ with the preference relations $\preceq_W$ and $\preceq_W^{-1}$. Therefore, there is no winning strategy for the winning set $W$ among strategies implemented with memory skeleton $\mathcal{M}$.

	Now, assume that both $\preceq_W$ and $\preceq_W^{-1}$ are $\mathcal{M}$-monotone and $\mathcal{M}$-selective. First, note that $\preceq_W^{-1} = \preceq_{\colSet^\omega \setminus W}$, $\preceq_{W^\Aconc}^{-1} = \preceq_{\colSetSeq^\omega \setminus W^\Aconc}$, and $\colSetSeq^\omega \setminus W^\Aconc = (\projec{\colSetSeq}{\colSet})^{-1}[\colSet^\omega \setminus W]$. If follows, by Theorem~\ref{thm:winning_condition_stability}, that $\preceq_{W^\Aconc}$ and $\preceq_{W^\Aconc}^{-1}$ are $\mathcal{M}^\Aconc$-monotone and $\mathcal{M}^\Aconc$-selective. Furthermore, since the concurrent game $\Aconc$ is finite, its sequential version $\ATurnConc$ also is. Thus, by Theorem~\ref{thm:turn_equiv_memory_winning}, the sequential version $\ATurnConc$ of the concurrent game $\Aconc$ is determined for $W^\Aconc$ and there exists a winning strategy implemented with the memory skeleton $\mathcal{M}^\Aconc =  \langle M,m_{init},\trT(\mu) \rangle$. Then, with Lemma~\ref{lem:turn_to_conc_memory}, we deduce that there exists a winning strategy $\s$ in $\Aconc$ for $W$ implemented with the memory skeleton $\langle M,m_{init},\trC(\trT(\mu)) \rangle$. Finally, note that for all $m \in M$ and $k \in \colSet$, we have $\trC(\trT(\mu))(m,k) = \trT(\mu)((\trT(\mu),k_\Aconc),k) = \trT(\mu)(m,k) = \mu(m,k)$. That is, $\trC(\trT(\mu)) = \mu$. In fact, the winning strategy $\s$ can be implemented with the memory skeleton $\mathcal{M}$.
\end{proof}

Overall, we obtain, in locally determined concurrent games, the same
equivalence that the authors of \cite{DBLP:conf/concur/Bouyer0ORV20} proved in 
turn-based games: every finite game is determined for $W$ with memory skeleton 
$\mathcal{M}$ if and only if $\preceq_{W}$ and $\preceq_{W}^{-1}$ are 
$\mathcal{M}$-monotone and $\mathcal{M}$-selective. In addition, we also have 
that the local determinacy assumption is somehow a necessary condition in the 
sense that as soon as concurrent games are built on at least one local 
interactions that is not determined, the aforementioned equivalence does not 
hold anymore. Formally, we have the following theorem:
\begin{theorem}
	Consider a set of game forms $\mathcal{I}$, and a set of colors $K$ with $|K| > 1$. Then the following assertions are equivalent:
	\begin{itemize}
		\item[1.] $\mathcal{I} \subseteq \allDet$; 
		\item[2.] For all memory skeleton $\mathcal{M}$, for all set $W \subseteq K^\omega$, the following assertions are equivalent:
		\begin{itemize}
			\item $\preceq_{W}$ and $\preceq_{W}^{-1}$ are 
			$\mathcal{M}$-monotone 
			and $\mathcal{M}$-selective;
			\item every finite concurrent game built on $\mathcal{I}$ is 
			determined for $W$ and there exists a winning strategy implemented 
			with memory skeleton $\mathcal{M}$;
		\end{itemize}
		\item[2'.] There exists a memory skeleton $\mathcal{M}$ such that for all set $W \subseteq K^\omega$, the following assertions are equivalent:
		\begin{itemize}
			\item $\preceq_{W}$ and $\preceq_{W}^{-1}$ are 
			$\mathcal{M}$-monotone 
			and $\mathcal{M}$-selective;
			\item every finite concurrent game built on $\mathcal{I}$ is determined for $W$ and there exists a winning strategy implemented with memory skeleton $\mathcal{M}$.
		\end{itemize}
	\end{itemize}
\end{theorem}
\begin{proof}
	Implication $(1) \Rightarrow (2)$ comes from 
	Theorem~\ref{thm:conc_equiv_memory_winning}, implication $(2) \Rightarrow 
	(2')$ is straightforward. As for implication $(2') \Rightarrow (1)$, 
	consider a memory skeleton $\mathcal{M}$ and a reachability objective $W$, 
	with $\colSet^\omega \setminus W$ a safety objective. Then, both of those 
	kind of objectives can be solved with positional strategies 
	\bbcomment{(ref?)}. Since positional strategies can be implemented by any 
	memory skeleton, in particular it can be implemented with $\mathcal{M}$. 
	Then, by Theorem~\ref{thm:turn_equiv_memory_winning}, it follows that 
	$\preceq_W$ and $\preceq_W^{-1} = \preceq_{\colSet^\omega \setminus W}$ are 
	$\mathcal{M}$-monotone and $\mathcal{M}$-selective. Now, if $\mathcal{I} 
	\subsetneq \allDet$, a finite concurrent game with an initial interaction 
	that is not determined that can either reach the desired color or not is 
	built on $\mathcal{I}$ and is not determined for $W$ which contradicts 
	$(2')$. It follows that $(2') \Rightarrow (1)$.
\end{proof}






==> Tex/NashEq.tex <==
%Application resultat stephane
A direct application of the results we have established in this paper lies in the existence of Nash equilibria. In \cite{DBLP:journals/mlq/Roux14}, the author proved that the existence of winning strategies could be transferred to the existence of Nash equilibria. That is, consider a colored concurrent graph arena $\Aconc = \AcoloredConc$ and a set $\mathcal{D} \subseteq 2^{\colSet^\omega}$ of subsets of outcomes that forms a partition of the set $\colSet^\omega$: $\colSet^\omega = \uplus_{D \in \mathcal{D}} D$ along with two preference relations $\prec_\A \subseteq \mathcal{D} \times \mathcal{D}$ and $\prec_\B \subseteq \mathcal{D} \times \mathcal{D}$ respectively for Player $\A$ and Player $\B$\footnote{Note that this a generalization of win/lose game where we consider the special where $\mathcal{D} = \{ W,\colSet^\omega \setminus W \}$ for some $W \subseteq \colSet^\omega$ and $\prec_\A^{-1} = \prec_\B$.}. Informally, a Nash equilibrium consists in a pair of strategies where no player has an interest (with regard to his preference relation) in unilaterally changing his strategy. That is, if for a pair of strategies $(\s_\A,\s_\B) \in \SetStrat{\Aconc}{\A} \times \SetStrat{\Aconc}{\B}$, we denote by $\delta(\s_\A,\s_\B)$ the unique path in $\OutStrat{\Aconc}^\omega(\s_\A) \cap \OutStrat{\Aconc}^\omega(\s_\B)$, we have the following definition:
\begin{definition}
	A pair of strategies $(\s_\A,\s_\B) \in \SetStrat{\Aconc}{\A} \times \SetStrat{\Aconc}{\B}$ is a \emph{Nash equilibrium} if, for all strategy $\s \in \SetStrat{\Aconc}{\A}$ (resp. $\SetStrat{\Aconc}{\B}$), we have that $\delta(\s_\A,\s_\B) \prec_\A \delta(\s,\s_\B)$ (resp. $\delta(\s_\A,\s_\B) \prec_\B \delta(\s_\A,\s)$) does not hold.
\end{definition}

Then, the following theorem is directly derived from Theorem 1.7 in \cite{DBLP:journals/mlq/Roux14}.
\begin{theorem}
	Consider a concurrent arena $\Aconc = \AcoloredConc$, a partition $\mathcal{D} \subseteq 2^{\colSet^\omega}$ of $\colSet^\omega$, two preference relations $\prec_\A,\prec_\B \subseteq \mathcal{D} \times \mathcal{D}$, and two subsets of strategies $R_\A \subseteq \SetStrat{\Aconc}{\A}$ and $R_\B \subseteq \SetStrat{\Aconc}{\B}$
	and assume the following:
	\begin{itemize}
		\item for all $\mathcal{H} \subseteq \mathcal{D}$, the win/lose game $\langle \mathcal{C},W \rangle$ is determined for $W = \uplus_{H \in \mathcal{H}} H$ with winning strategies in $R_\A$ or $R_\B$;
		\item the preference $\prec_\A$ (resp. $\prec_\B$) has finite height, that is there exists $n \in \mathbb{N}$ such that there is no $D_1,D_2, \ldots, D_n \in \mathcal{D}$ such that $D_1 \prec_\A D_2 \prec_\A \ldots \prec_\A D_n$.
	\end{itemize}
	Then, there exists a Nash equilibrium in $\mathcal{C}$ with the preference relations $\prec_\A$ and $\prec_\B$ that can be found in $R_\A \times R_\B$.
	\label{thm:nash_existence}
\end{theorem}

\paragraph*{Application: Nash equilibrium with Borel outcomes} By combining Theorem~\ref{thm:nash_existence} and Corollary~\ref{coro:conc_borel_determined}, we obtain the following theorem:
\begin{theorem}
	Consider a concurrent arena $\Aconc = \AcoloredConc$, a partition $\mathcal{D} \subseteq 2^{\colSet^\omega}$ of $\colSet^\omega$, two preference relations $\prec_\A,\prec_\B \subseteq \mathcal{D} \times \mathcal{D}$ and assume the following:
	\begin{itemize}
		\item $\mathcal{D}$ is countable and all sets $D$ of $\mathcal{D}$ are Borel;
		\item the preference $\prec_\A$ (resp. $\prec_\B$) has finite height.
	\end{itemize}
	Then, there exists a Nash equilibrium in $\mathcal{C}$ with the preference relations $\prec_\A$ and $\prec_\B$.
	\label{thm:nash_existence_conc_borel}
\end{theorem}

\paragraph*{Application: Nash equilibrium in a priority game}
By combining Theorem~\ref{thm:nash_existence}, Theorem~\ref{thm:determinacy_equivalence_memory}, and the fact that turn-based parity games are positionally determined (see for instance \cite{DBLP:conf/focs/EmersonJ91,mostowski1991games,zielonka1998infinite}), we obtain the following theorem:
\begin{theorem}
	Consider a finite concurrent arena $\Aconc = \AcoloredConc$ where $\colSet = \llbracket 0,n \rrbracket$ for some $n \in \mathbb{N}$. For all $k \in \colSet$, we define $D_k = \{ \rho \in \colSet^\omega \mid \max (\inf \rho) = k \}$ where $\inf \rho$ is the set of colors seen infinitely often in $\rho$. Consider $\mathcal{D} = \{ D_k \mid k \in \colSet \}$ and two preference relations $\prec_\A,\prec_\B \subseteq \mathcal{D} \times \mathcal{D}$ and assume that  the preferences $\prec_\A$ and $\prec_\B$ are acyclic.
	
	Then, there exists a Nash equilibrium in $\mathcal{C}$ with the preference relations $\prec_\A$ and $\prec_\B$ among positional strategies.
	\label{thm:nash_existence_conc_priority}
\end{theorem}



